Living in Parallel Realities -- Co-Existing Schema Versions with a Bidirectional Database Evolution Language

We introduce end-to-end support of co-existing schema versions within one database. While it is state of the art to run multiple versions of a continuously developed application concurrently, it is hard to do the same for databases. In order to keep multiple co-existing schema versions alive; which are all accessing the same data set; developers usually employ handwritten delta code (e.g. views and triggers in SQL). This delta code is hard to write and hard to maintain: if a database administrator decides to adapt the physical table schema, all handwritten delta code needs to be adapted as well, which is expensive and error-prone in practice. In this paper, we present InVerDa: developers use the simple bidirectional database evolution language BiDEL, which carries enough information to generate all delta code automatically. Without additional effort, new schema versions become immediately accessible and data changes in any version are visible in all schema versions at the same time. InVerDa also allows for easily changing the physical table design without affecting the availability of co-existing schema versions. This greatly increases robustness (orders of magnitude less lines of code) and allows for significant performance optimization. A main contribution is the formal evaluation that each schema version acts like a common full-fledged database schema independently of the chosen physical table design.

==> chapters/5_bidirectionality.tex <==
In the following we sketch our approach to formally show bidirectionality for all \indel SMOs.
Basically, we have to show that the two bidirectionality conditions (Rule~\ref{align:ds} and Rule~\ref{align:dt}) hold.
Given data in one schema version, mapping it through the SMO to another schema version, and mapping it back again should always result in the originally given data.
For brevity, we show this for one condition (Rule~\ref{align:ds}) of the split/merge SMO in detail and would like to direct the curious reader to our technical report~\cite{Herrmann2016}, where we formally show the bidirectionality of all \indel operations in detail.

Given data in the source database \ds map it through the split SMO to the target database \dt and back again.
To formally show that the result is equal to the originally given data, hence $\ds=\getSource(\getTarget(\ds))$ holds, we follow two basic steps.
First, we reduce $\getTarget(\ds)$, since data in \ds is exclusively represented in the source \contabs.
There are no \auxtabs necessary.
Second, we take the results of reducing $\getTarget(\ds)$ as input for $\getSource$ and show that we obtain exactly the initial data \ds.
The same process applies to the other direction.

Reducing sets of Datalog rules is the central task.
So, we present six lemmas which describe typical equivalence transformations for our specific sets of Datalog rules.
Let $RB$ be a rule body, $RH$ a rule head, and $Var(RL)$ the set of all variables in the set of literals $RL$.

\begin{lemma}[Empty Literal]\label{lemma:empty}
Let $L$ be a literal in $RB$ that is empty.
We can remove the whole rule if $L$ is a positive literal or remove $L$ from $RB$ if $L$ is negated.
\end{lemma}
\begin{lemma}[Application]\label{lemma:projection}
Given a rule $RH \leftarrow RB_1, B(X,\_)$ we can replace it with $RH \leftarrow RB_1, RB_n$ for each rule $B(X,Y) \leftarrow RB_n$.
All attributes in $RB_n$ except of $X$ that also occur in $RH$ and $RB_1$ need to be renamed, so that $(Var(RB_n)\setminus X)\cap(Var(RB_1)\cup Var(RH))=\emptyset$.
%Let $X$ be a set of variables such that $Var(RB_1) \cap Var(RH)\subseteq {X}$.
%Then, applying a rule $B(X,Y) \leftarrow RB_1$ to a rule $RH \leftarrow RB_2, B(X,\_)$ is the same as applying the rule $RH \leftarrow RB_2,RB_1$. 
%If the presumption is not met, shared variables can be renamed.\\
Note: Applying a rule $RH(p,A) \leftarrow \neg R(p,A)$ with $R(p,A) \leftarrow B1(p1,A1),B2(p2,A2)$, we would obtain the rule
$RH(p,A) \leftarrow \neg(B1(p1,A1),B2(p2,A2))$, which is no valid Datalog syntax. 
The following lemma states how to cope with this problem.
\end{lemma}
\begin{lemma}[De Morgan's laws]\label{lemma:morgan}
Given a rule $RH(X_0) \leftarrow RB, \neg(R_1(X_1),...,R_n(X_n))$ we can replace this rules with this set of rules:
\begin{align*}
RH(X_0) &\leftarrow RB, \neg R_1(X_1)\\[-2mm]
\vdots&\\
RH(X_0) &\leftarrow RB, \neg R_n(X_n)
\end{align*}
\end{lemma}
\begin{lemma}[Functional Dependency]\label{lemma:p}
Whenever we have two literals $A(\pk,X)$ and $A(\pk,Y)$, we can assume $X=Y$ due to the common key \pk.
\end{lemma}
\begin{lemma}[Tautology]\label{lemma:tautology}
Given two rules $RH \leftarrow RB,C(X)$ and $RH\leftarrow RB,\neg C(X)$, we can replace these rules with $RH \leftarrow RB$.\\
Note: This is true since $C(X) \vee \neg C(X) = \top$
\end{lemma}
\begin{lemma}[Unsatisfiability]\label{lemma:unsatisfiability}
Given a rule with $RH \leftarrow RB,C(X),\neg C(X)$, we can remove this rule.
\end{lemma}

\subsection{Split and Merge}
We already introduced the Datalog rules describing the split SMO in detail.
\begin{align*}
&\sql{\sqlk{\PARTITION TABLE} $T$ \sqlk{INTO} $R$ \sqlk{WITH} \cR, $S$ \sqlk{WITH} \cS}
\end{align*}
We will now show bidirectionality for this SMO using the rule set discussed in Section~\ref{sec:architecture}:
\begin{align}
\mathbf{\getTarget:}\phantom{T(\pk,A)}&\nonumber\\
R(\pk,A)&\leftarrow T(\pk,A),\cR (A), \neg R^-(\pk)\\
S(\pk,A)&\leftarrow T(\pk,A),\cS (A), \neg S^-(\pk), \neg S^+_\pk(\pk)\\
S(\pk,A)&\leftarrow S^+(\pk,A)\\
T'(\pk,A)&\leftarrow T(\pk,A),\neg \cR (A),\neg \cS (A)\\
\mathbf{\getSource:}\phantom{T(\pk,A)}&\nonumber\\
T(\pk,A)&\leftarrow R(\pk,A)\\
T(\pk,A)&\leftarrow S(\pk,A), \neg R_\pk(\pk)\\
T(\pk,A)&\leftarrow T'(\pk,A)\\
S^+(\pk,A)&\leftarrow S(\pk,A), R(\pk,A'),A\neq A'\\
S^-(\pk) &\leftarrow R(\pk,A),\neg S_\pk(\pk),\cS (A)\\
R^-(\pk) &\leftarrow S(\pk,A),\neg R_\pk(\pk),\cR (A)
\end{align}

The first step to formally show bidirectionality is to assume data in the source schema table $\Tdata$ and map it to the target schema.
For data stored at the source schema, the \auxtabs $S^+$, $S^-$, and $R^-$ are not necessary, hence we assume them to be empty.
Using Lemma~\ref{lemma:empty}, we immediately eliminate the rules having one of these tables as positive literal and reduce the rules having a negative literal on one of them.
The reduced rule set for reading data $T_D$ from \ds to \dt is
\begin{align}
\mathbf{\getTarget(\Tdata):}&\nonumber\\
R(\pk,A)&\leftarrow \Tdata(\pk,A),\cR (A)\\
S(\pk,A)&\leftarrow \Tdata(\pk,A),\cS (A)\\
T'(\pk,A)&\leftarrow \Tdata(\pk,A),\neg \cR (A),\neg \cS (A)
\end{align}
The above rule set describes how to transform the source data according to the target schema version.
To show bidirectionality we transform the data back and show that it survives the round trip completely and correctly without any information loss or gain.
For that purpose we insert the rule bodies of $\getTarget(\Tdata)$ into $\getSource$ following Lemma~\ref{lemma:projection}, which result in the following rule set:
\begin{align}
\noalign{$\mathbf{\getSource(}\mathbf{\getTarget(\Tdata)):}$}
T(\pk,A)&\leftarrow \Tdata(\pk,A),\cR (A)\\
T(\pk,A)&\leftarrow \Tdata(\pk,A),\cS (A), \neg (\Tdata(\pk,A),\cR (A))\label{align:t}\\
T(\pk,A)&\leftarrow \Tdata(\pk,A),\neg \cR (A),\neg \cS (A)\\
S^+(\pk,A)&\leftarrow \Tdata(\pk,A),\cS (A), \Tdata(\pk,A'),\nonumber\\
\phantom{S^+(\pk,A)}&\phantom{\leftarrow }\cR (A'), A\neq A'\label{align:splus}\\
S^-(\pk) &\leftarrow \Tdata(\pk,A),\cR (A),\nonumber\\
\phantom{S^-(\pk) }&\phantom{\leftarrow }\neg (\Tdata(\pk,A),\cS (A)),\cS (A)\label{align:smius}\\
R^-(\pk) &\leftarrow \Tdata(\pk,A),\cS (A),\nonumber\\
\phantom{R^-(\pk) }&\phantom{\leftarrow }\neg (\Tdata(\pk,A),\cR (A)),\cR (A)\label{align:rminus}
\end{align}
To finally show the bidirectionality, we reduce these rules.
Let us start with the rules, producing $T(\pk,A)$.
By applying De Morgan's laws (Lemma~\ref{lemma:morgan}), we resolve the negation in Rule~\ref{align:t} and split it into two new rules, which leads to the following rules $T$:
\begin{align}
T(\pk,A)&\leftarrow \Tdata(\pk,A),\cR (A)\label{align:pr1}\\
T(\pk,A)&\leftarrow \Tdata(\pk,A),\cS (A), \neg \Tdata(\pk,A) \label{align:partition_Source_T_empty}\\
T(\pk,A)&\leftarrow \Tdata(\pk,A),\cS (A), \neg \cR (A)\label{align:ps}\\
T(\pk,A)&\leftarrow \Tdata(\pk,A),\neg \cS (A), \neg \cR (A) \label{align:ns}
\end{align}
According to Lemma~\ref{lemma:unsatisfiability}, Rule~\ref{align:partition_Source_T_empty} will never add data to $T$, since there are two conflicting conditions $\Tdata(\pk,A)$ and $\neg \Tdata(\pk,A)$.
The remaining rules can be reduced by applying Lemma~\ref{lemma:tautology}.
We combine Rule~\ref{align:ps} and Rule~\ref{align:ns} to Rule~\ref{align:nr}, since $c_S(A)$ occurs both as positive and negative literal respectively.
So, we reduced Rules~\ref{align:pr1}-\ref{align:ns} to:
\begin{align}
T(\pk,A)&\leftarrow \Tdata(\pk,A),\cR (A)\label{align:pr2}\\
T(\pk,A)&\leftarrow \Tdata(\pk,A),\neg \cR (A) \label{align:nr}
\end{align}
Rules~\ref{align:nr} and~\ref{align:pr2} can be reduced following to same principle.
So, finally we obtain the following for $T$:
\begin{align}
T(\pk,A)&\leftarrow \Tdata(\pk,A) \label{partition_Source_T_logic_final}
\end{align}
%Let us continue with the remaining Rules~\ref{align:splus}-\ref{align:rminus}.
Rule~\ref{align:splus} for $S^+$ reduces to $S^+(\pk,A)\leftarrow \emptyset$ since \pk uniquely identifies $A$  (Lemma~\ref{lemma:p}) and it is impossible that there are different values for $A$ for the same \pk:
\begin{align}
S^+(\pk,A)&\leftarrow \emptyset
\end{align}
The Rules~\ref{align:smius} and~\ref{align:rminus} for $S^-$ and $R^-$ can be replaced using De Morgan's laws (Lemma~\ref{lemma:morgan}) to obtain the following:
\begin{align}
S^-(\pk) &\leftarrow \Tdata(\pk,A),\cR (A),\neg \Tdata(\pk,A),\cS (A)\\
S^-(\pk) &\leftarrow \Tdata(\pk,A),\cR (A),\neg \cS (A),\cS (A)\\
\nonumber\\
R^-(\pk) &\leftarrow \Tdata(\pk,A),\cS (A),\neg \Tdata(\pk,A),\cR (A)\\
R^-(\pk) &\leftarrow \Tdata(\pk,A),\cS (A),\neg \cR (A),\cR (A)
\end{align}
In each rule, there are contradicting literals on \Tdata, \cR, and \cS respectively.
Lemma~\ref{lemma:unsatisfiability} reduces these rules to the final rule set for $\getSource(\getTarget(\Tdata))$:
\begin{align}
T(\pk,A)&\leftarrow \Tdata(\pk,A)\\
S^+(\pk,A)&\leftarrow \emptyset\\
S^-(\pk) &\leftarrow \emptyset\\
R^-(\pk) &\leftarrow  \emptyset \qed
\end{align}
This formally shows that data from the source schema can be stored at the target schema and translated back without any information loss or gain.
The same condition holds for the other direction, which we do not deduce in detail here, but directly present the result:
\begin{align}
R(\pk,A)&\leftarrow \Rdata(\pk,A)\\
S(\pk,A)&\leftarrow \Sdata(\pk,A)\\
T'(\pk) &\leftarrow \emptyset
\end{align}
So, the data is never lost independently in which version it is written, stored, or read.
The merge operation is just the opposite of split, hence we would exchange \getTarget and \getSource to obtain its mapping rules resulting in essentially the same argument.

%\input{chapters/5_5_addColummnDecompose}
In our technical report~\cite{Herrmann2016}, we used the same method to show bidirectionality for all presented \indel operations.
This is a solid formal foundation for the forward and backward propagation of read and write accesses among multiple co-existing schema versions independently of the actual materialization.
Starting with established DELs, we defined \indel and formally showed that all \indel operations are bidirectional.
So, given data at any schema version $V_n$ which is propagated and stored at another schema version $V_{n+1}$, we can always read the initial data completely and correctly at schema version $V_n$.
